Exploring the Advances in Using Machine Learning to Identify Technical Debt and Self-Admitted Technical Debt

In software engineering, technical debt, signifying the compromise between short-term expediency and long-term maintainability, is being addressed by researchers through various machine learning approaches. This study seeks to provide a reflection on the current research landscape employing machine learning methods for detecting technical debt and self-admitted technical debt in software projects and compare the machine learning research about technical debt and self-admitted technical debt. We performed a literature review of studies published up to 2024 that discuss technical debt and self-admitted technical debt identification using machine learning. Our findings reveal the utilization of a diverse range of machine learning techniques, with BERT models proving significantly more effective than others. This study demonstrates that although the performance of techniques has improved over the years, no universally adopted approach reigns supreme. The results suggest prioritizing BERT techniques over others in future works.

==> sec_related_work.tex <==
\section{Related Work}

Below you can see find studies discussing TDM, a multi-level view of handling TD.  Unlike our paper which focuses the advancements of using ML techniques for SATD identification and its differences from TD identification, the following studies provide reviews of research on TDM activities including: identification, prediction, measurement, prioritization, prevention, monitoring, repayment, representation, and communication.

Li et al. ~\cite{li_systematic_2015} performed a systematic mapping study on technical debt and its management.  In the study, they make classification and thematic analyses based on 94 studies between 1992 and 2013.  The result is TD classification into 10 types, 8 TDM activities, and 92 tools for TDM. 

Tsintzira et al.~\cite{tsintzira2020applying} analyzed ML across all TDM activities and found of current techniques 89\% are compromised of supervised learning algorithms, followed by unsupervised 6\%, and semi-supervised 5\%.  In regard to specifically TD identification, they reference 6 studies using Naive Bayes, 5 Random Forest, 5 C4.5, 4 AdaBoost, and 4 Support Vector Machines.  
They identified that Neural Network Analysis appears to be fitting for Cost and Effort Estimation practices, Bayesian Networks for Defect and Project Management practices, and Random Forrest algorithms appear to be appropriate for Managing Design-Time QAs. On the other hand, Clustering and Decision Trees appear to be equally fitting for various SE practices.  
They concluded that studies focusing on code smells, patterns and tactics detection are fitting for elaborate TD identification.

D. Albuquerque et al.~\cite{albuquerque_comprehending_2022} more recently a similar study but didn't limit their search to only ML approaches but to all intelligent techniques.  Across all intelligent techniques for TDM Machine Learning was used 47\% of the time. Based on this sample, approximately 55\% of the solutions used supervised learning techniques, such as regression analysis (35\%), neural networks (19\%), and support vector machines (6\%). The rest of the machine learning techniques used comprised of tree techniques (35\%), and clustering techniques (6\%). Interestingly, from their study they reported that across all TDM activities TD identification was covered by 79\% of studies, showing that TD identification is heavily prioritized over other types of TDM activities. 

On the other hand, extending upon the created frameworks and tools touched on by the objective column of Table~\ref{tab:comparison}), there is plenty of ongoing work in the research community to develop tools to increase the number of TD items for analysis in order to derive more robust conclusions and find new approaches and behaviors, such as Sonarlizer Xplorer~\cite{pina_sonarlizer_2022}, and Jitterbug~\cite{yu_identifying_2022}.

Sonarlizer Xplorer~\cite{pina_sonarlizer_2022} is an open source tool which uses SonarQube behind the hood. This tool can be used for identifying a massive number of TD items and code metrics from public GitHub repositories and can remedy the requirement of establishing a large amount of data in order to apply ML methods for future researchers. It should be considered applying in future research related to TD/SATD identification.

Jitterbug~\cite{yu_identifying_2022}, is a framework with two methods for identifying SATD in software systems. The first method classifies ``easy to find'' TD, which is capable of finding 0.20-0.90 of SATD automatically without any human intervention. The second method, ``hard to find,'' is a method in which practitioners must intervene to make the final decision on an item being TD or not. Jitterbug is the first instance of reviewed literature which breaks up SATD in two categories, which may also prove to be a promising direction for future research to take.

%As Sonarlizer Xplorer and Jitterbug show, extending upon the current state-of-the-art tools and classifying TD into ``easy'' and ``hard'' can be two exciting avenues for future researchers to explore.
